Letter of Intent: Open Charm at JLab with the sPHENIX MAPS tracker

We propose a physics program at JLab with CLAS12 focusing on open-charm measurements, aiming to complement and expand current studies of $J/\psi$ at (sub) threshold. This program will aid us in elucidating the $J/\psi$ production mechanisms, which is crucial for interpreting data in terms of gluon form factors and offer potential insights into the intrinsic charm hypothesis and cold-nuclear matter effects. We discuss the technical feasibility of integrating the sPHENIX monolithic-active-pixel sensor (MAPS) tracker, known as MVTX, with the CLAS12 detector. The sPHENIX MTVX would support an open-charm program by providing excellent secondary-vertex performance for tagging $D$ mesons. We study the kinematics of $\gamma p \to \bar{D}^{0}\Lambda_{c}$ through phase-space simulations and estimate rates for the tagged quasi-photoproduction regime available with the CLAS12 forward tagger. While open-charm cross-sections at threshold remain uncertain, various predictions suggest that these measurements could be feasible when combined with conservative estimates of detector acceptance and luminosity. These preliminary estimates motivate detailed Geant detector simulations of signals and backgrounds, along with thorough technical assessments of operating conditions, to further explore the feasibility of these measurements in future dedicated CLAS12 experiments at JLab.

==> ExpectedPerformance.tex <==
\section{Expected Performance}

\subsection{Geometric acceptance of the MVTX in CLAS12}
If the upstream end of the MVTX is aligned with the target, as shown in Fig.~\ref{fig:sketchup3d}, then the MVTX would be able to measure as low as 8.7$^\circ$.  In principle, determining the decay position of a charmed hadron requires at least one of its decay products to be within the acceptance of the detector.  However, as an alternative to reduce backgrounds from poorly reconstructed single tracks, it is possible to require at least two of the decay products to be reconstructed in the MVTX.

We show the overall geometric acceptance of the MVTX (that is the fraction of the generated events which a requisite number of the decay products are in the MVTX's geometric acceptance) of these scenarios in Fig.~\ref{fig:MVTX_acceptance}.  
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/MVTX_acceptance.pdf}
    \caption{Overall geometric acceptance of }
    \label{fig:enter-label}
\end{figure}


\subsection{Foil thickness}
To determine how the thickness of the target would affect the efficiency of a displaced-vertex cut, we used the event-generator simulations described in Sec. XXX.  In this exercise, we choose to use a cut on $v_z$ at 15 $\mu$m (approximately 3$\sigma$) from the downstream face of the target foil.  The efficiency of this cut can be calculated as:
\begin{equation}
    \epsilon_h(v_{z,\rm cut})=\frac{N(v^h_z>v_{z,\rm cut})}{N_{\rm tot}}
    
\end{equation}
where $N(v_z>v_{z,\rm cut})$ is the number of events where the decay position of one of the charmed hadrons, $v^h_z$, (where the $h$ index represents either $\Lambda_c^+$ or $\bar D^0$), is greater than the cutoff, $v_{z,\rm cut}$.  The $v^h_z$ for each event is given by 
\begin{equation}
    v^h_z= v^{h,\rm gen}_z+v^e_z
\end{equation}
where $v^{h,\rm gen}_z$ is the $z$ position of the charmed-hadron decay from the event generator ($i.e.$, relative to the electron vertex), and $v^e_z$ is the electron vertex, which assigned uniformly to each event between $-t$ and $0$, where $t$ is the thickness of the foil.  

The resulting cut efficiency, as a function of the foil thickness, is shown in Fig.~\ref{fig:vertex_cut_efficiency}. 
 We note that with a foil that is a few tens of microns thick, the efficiency of this cut is sufficiently thin: 
 with a 50 $\mu$m foil, at least 75\% of $\Lamba_c^+$s and 86\% of $\bar D^0$s decay after the cutoff.  

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/vertex_cut_efficiency.pdf}
    \caption{Efficiency for a displaced-vertex cut at 15~$\mu$m for the $\Lambda_c^+$ (blue) and $\bar D_0$ (orange) channels respectively}
    \label{fig:vertex_cut_efficiency}
\end{figure}



==> Figures/PossibleExp.tex <==
\section{Possible experiments with CLAS12 and sPHENIX MVTX}

Here we discuss possible targets and trigger strategies for experiments with CLAS12 and the sPHENIX MVTX.

As we showed in Section~\ref{fig:MVTX}, the possible experiments using both CLAS12 and sPHENIX MVTX require to remove the vacuum scattering chamber that normally encapsulates a cryotarget to make space for the MVTX detector and its services. Instead of having a cryotarget, we will use a solid target setup, which would be smaller and much simpler.  

Practically, the lightest solid target could be beryllium. Other heavier targets could be carbon or even heavier targets. Such heavier targets were used in the CLAS12 run-group D ``color transparency'' experiments at high energy, and are scheduled to run in the CLAS12 run-group E ``hadron-formation'' experiments. Similar strategies could be pursued in these experiments, but 

Possible triggers could be implemented using the forward tagger, which was designed to measure small-angle scattering to access the the small-$Q^{2}$ regime of electro-production ($0.01<Q^{2}<0.1$). 

==> PossibleExp.tex <==
\section{Possible experiments with CLAS12 and sPHENIX MVTX}

Here we discuss possible targets and trigger strategies for experiments with CLAS12 and the sPHENIX MVTX.

As we showed in Section~\ref{fig:MVTX}, the possible experiments using both CLAS12 and sPHENIX MVTX require to remove the vacuum scattering chamber that normally encapsulates a cryotarget to make space for the MVTX detector and its services. Instead of having a cryotarget, we will use a solid target setup, which would be smaller and much simpler.  

Practically, the lightest solid target could be beryllium. Other heavier targets could be carbon or even heavier targets. Such heavier targets were used in the CLAS12 run-group D ``color transparency'' experiments at high energy, and are scheduled to run in the CLAS12 run-group E ``hadron-formation'' experiments. Similar strategies could be pursued in these experiments, but 




Possible triggers could be implemented using the forward tagger, which was designed to measure small-angle scattering to access the the small-$Q^{2}$ regime of electro-production ($0.01<Q^{2}<0.1$). 



==> Sketchs.tex <==
\section{Possible experiments layout including the sPHENIX tracker}
The same geometry could be imported in the CLAS12 detector, provided the cryotarget is removed and a smaller solid target is used instead. For reference, the SVT inner-most layer is located at $r$=65 mm, with the SVT within a Faraday cage. 

\begin{figure}
    \centering
        \includegraphics[width=0.4\linewidth]{Figures/Sketchup3D.png}
    %\includegraphics[width=0.6\linewidth]{Figures/layout.png}
    \includegraphics[width=0.6\linewidth]{Figures/mvtx_two_views.pdf}
    \caption{Top: Rendering of possible layout of sPHENIX MVTX (cyan) with the CLAS12 SVT (green) and BMT (purple and orange). Bottom: Possible layout of the sPHENIX MVTX and the CLAS12 SVT and BMT. This configuration would be compatible with a solid-target.}
    \label{fig:sketchup3d}
\end{figure}
